An Extensible Dashboard Architecture For Visualizing Base And Analyzed Data

Any data analysis, especially the data sets that may be changing often or in real-time, consists of at least three important synchronized components: i) figuring out what to infer (objectives), ii) analysis or computation of objectives, and iii) understanding of the results which may require drill-down and/or visualization. There is a lot of attention paid to the first two of the above components as part of research whereas the understanding as well as deriving actionable decisions is quite tricky. Visualization is an important step towards both understanding (even by non-experts) and inferring the actions that need to be taken. As an example, for Covid-19, knowing regions (say, at the county or state level) that have seen a spike or prone to a spike in cases in the near future may warrant additional actions with respect to gatherings, business opening hours, etc. This paper focuses on an extensible architecture for visualization of base as well as analyzed data. This paper proposes a modular architecture of a dashboard for user-interaction, visualization management, and complex analysis of base data. The contributions of this paper are: i) extensibility of the architecture providing flexibility to add additional analysis, visualizations, and user interactions without changing the workflow, ii) decoupling of the functional modules to ease and speedup development by different groups, and iii) address efficiency issues for display response time. This paper uses Multilayer Networks (or MLNs) for analysis. To showcase the above, we present the implementation of a visualization dashboard, termed CoWiz++ (for Covid Wizard), and elaborate on how web-based user interaction and display components are interfaced seamlessly with the back end modules.

==> texFiles/abhishek.tex <==



\section{Integration of Different Front-End and Back-End Components}
\label{sec:arch-int}



==> texFiles/enamul.tex <==
In the top panel of the CoWiz dashboard, we can see the cumulative number of Covid cases and deaths in the United States and worldwide. The data required for the purpose is collected from the World Health Organization's (WHO) website. A \textbf{cron job} has been written on the Linux machine that hosts the dashboard to download the appropriate dataset periodically. Every time the dashboard's front page is opened, an \textbf{ajax script} is called to load the most recent csv file and calculate the overall number of cases and deaths in the United States and around the world. The result is then displayed on the top panel of the dashboard.

We have used the \textbf{New York Times API} to fetch the top 10 covid news articles from the target period and display them on the panel with the period highlights. The API provides us with the flexibility to search news based on any keyword specified. We have written a Python script that sends the API the start and end dates of the user-specified target period, the search query, the number of articles to fetch, and the type of materials to view. The API returns the necessary articles based on the inputs provided. Users can scroll through the different news headlines, and by clicking on one, they can read the full article on the New York Times website.

As an extension to our previous work, we have introduced the parameter based aggregate analysis where users have the option to select up to 5 different  states and two features. The total number of covid cases and deaths of the selected states are displayed along with the two separate graphs corresponding to the two selected features. We have used a dataset from the Centers for Disease Control and Prevention (CDC) for calculating the states cases. The entire calculation is done on the back-end using a python code. 

==> texFiles/integration.tex <==
\section{Integrating the Dashboard Modules}
\label{sec:integration}

In this section, we discuss the framework chosen along with the alternatives considered, efficient decision and information flow between the components and efficient storage mechanisms utilised in order to achieve integration of the independently developed modules of the system. %Further, we enlist the future extensibility and optimization opportunities in the system.

\noindent \underline{\textbf{Web Framework}}: For integration, we need to choose a framework that can support the functionalities of the different modules, allows seamless communication between them, is easy to use, has detailed documentation and strong open-source community for future development and extensions, and supports web deployment to increase the portability of the dashboard.

\begin{table}[h]
    \centering
    \vspace{-15pt}
    \begin{tabular}{|m{1.3cm}|m{2.2cm}|m{1.6cm}|m{2cm}|m{2.5cm}|m{2.2cm}|}
        \hline
         & \textbf{Minimalistic} & \textbf{Language} & \textbf{Plotly Compatibility} & \textbf{Documentation Available} & \textbf{Flexibility and Control}\\
         \hline
         \textbf{Flask} & \textit{Yes} & \textit{Python} & \textit{Yes} & \textit{Extensive} & \textit{High} \\
         \hline
         Django & No & Python & Limited & Extensive & Low\\
         \hline
         Vaadin & No & Java & No & Limited & Low \\
         \hline
    \end{tabular}
    \caption{Web Framework Alternative and Feature Comparison}
    \label{table:framework-alts}
    \vspace{-25pt}
\end{table}

Table \ref{table:framework-alts} lists the features of the widely used web frameworks. The \textbf{python-based web framework Flask} has been chosen over Django and Vaadin, majorly due to its minimalistic, interactive, flexible and extensible nature. Flask ticks all the requirements listed above. Moreover, visualization tools like Plotly are supported in Flask, which is not supported in others. Most importantly, as compared to others, it gives maximum flexibility and control due to granular tuning for customisation and makes no assumptions about how data is stored, thus making a viable choice for a wider spectrum of applications. Flask's compatibility with Plotly made it the more desirable option when moving forward with the project.

\vspace{5pt}

\noindent \underline{\textbf{Decision and Information Flow between Components}}: The interactive flow between the different components is supported in the following manner.
\begin{enumerate}
    \item The user input parameters are passed on to from the client side to the back-end \textit{decision module}.
    \item The \textit{hash-index} is searched to check whether the desired visualization is already present. If present, then it is returned to the client-side and displayed on the dashboard front-end. If not present, then the user input parameters are passed on to the pre-processing module.
    \item Once the desired layers or cleaned files are generated using the input parameters, a \textit{configuration file} is prepared specifying the analysis expression and passed on to the analysis module.
    \item Based on the expression, the analysis results are generated only if they are not already stored (searched through the \textit{hash-index}). These results are passed on the visualization module.
    \item Finally, the HTML page with the desired visualization is returned to the client-side for display.
    \item This process continues for every set of user inputs.
\end{enumerate}


\vspace{5pt}

\noindent \underline{\textbf{Ease of Extensions}}: The modular analysis and visualization has multiple benefits from future extensibility point of view.
\begin{itemize}
    \item The \textbf{independence of back-end components} allows easy adding multiple front ends to the dashboard accepting different types of inputs. For instance, for the COVID visualization we are currently making use of two front-ends (for Category II and III objectives) that use the same back-end.
    \item Moreover, the new analysis and visualization tools can be easily added to the respective, making it \textbf{extensible} in nature.
    \item \textbf{Diverse data sets} and different analysis requirements can be \textbf{readily incorporated} to build interactive dashboards. We have plans to re-using the architecture for analysing accident, DBLP and IMDb data sets.
    \item The \textbf{hashing mechanisms} in the analysis and visualizations can be re-used for \textbf{efficiency aspects}.
    \item \textbf{Multi-threading} can be implemented for supporting multiple users, \textbf{increasing throughput}.
    \item \textbf{Efficient handling of access to critical sections} (hash-indexes) can lead to \textbf{improving the response time}.
\end{itemize} 
%iv) parameterization of back end to serve multiple front ends,

%vi) synchronization (critical sections) so the data generated at the back end is consistent


\begin{comment}


\textbf{Alternatives:} 

\tab As mentioned earlier, the team used Flask as the main framework to implement the features of CoWiz. During initial research, we discovered interesting frameworks which could have potentially helped us, including, Vaadin, Django, and Flask. Flask was preferred over the other similar frameworks as it was beneficial for various reasons. 

\tab Vaadin is a web framework which uses Java as the main programming language. It has the ability to create the user interface (UI) completely in Java without the use of external libraries, such as swing. However, this framework is not suitable to develop an interactive interface as we desired. 

\tab The second option we researched was Django. Django is a high level Python framework which is secure and allows for rapid web development. It is compatible with HTML, CSS, and Javascript and has libraries to aid visualisation. However, the downside to using Django was its incompatibility with Plotly, as well as its complicated nature as compared to Flask. 

\tab Flask is a minimalist python-based framework which is compatible with the required tools for the dashboard.

\tab Our next priority was to find an application or library that can be utilized by the Flask server to generate a choropleth map of the United States with the change in infection rates on a county-by-county basis.

\textbf{Challenges Encountered:}

\tab Over the course of designing and developing the project, we encountered a few challenges. These challenges include:

\begin{enumerate}
\item Connecting the framework to the Adobe web server.
\item Configuring the project to push to the Paris server. 
\end{enumerate}

\end{comment}

\begin{comment}


\sharma{4/3/21}{revised}
\begin{enumerate}
\item what is generated by analysis
\item how to transform it for visualization
\item Extensible approach to integrate the two. noting that they have been developed individually
\item challenges and efficiency issues (caching and hashing)
\item how efficiency can be improved further by generating results thru a script (using cycles when they are available)
\item interfacing the two
\item Extending each side individually
\item Examples of re-purposing with other data sets (with minimal changes). can use accident or airlines or DBLP data set
\item combined architecture
\end{enumerate}

\end{comment}




==> texFiles/kunal.tex <==
add table

1 state and 2 features 
5 states and 2 features 

==> texFiles/preprocessor.tex <==
\subsection{Pre-Processing and Storage Module (Dashboard Back-End Part)}
\label{sec:arch-pre}

%The data pre-processing module is hosted on the data server at the back-end of the dashboard.
This module has been divided into three separate sub-modules based on the different data pre-processing stages - data scrapping and collection, data cleaning, and data modeling. Covid-19 specific details have been discussed below.

\noindent \underline{\textbf{Data Scrapping and Collection}}: The first stage of data pre-processing involves the collection of data sets from various sources. The sub-module supports this  through (i) \textit{web scrapping} to download and extract data from online portals periodically, which are implemented through \textit{scheduled cron jobs} and ii) manual uploading of data sets. For CoWiz, \textit{periodic cron jobs} have been scheduled to extract US States data - (\textbf{D1}) Daily Covid-19 Data, reported by Centers for Disease Control (CDC) \cite{}, \textbf{(D2)} Daily Covid-19 Vaccinations Data \cite{}, (\textbf{D3}) Daily Trips by Distance Data, reported by US Department of Transportation \cite{}, (\textbf{D4}) Daily Community Mobility Reports in Different Categories of Places, Reported by Google \cite{}, (\textbf{D5}) New York Times News Articles (using API \cite{}) and (\textbf{D6}) New York Times Covid Data Repository for US Counties \cite{}. Moreover, the (\textbf{D7}) US Census data \cite{} is also available.
    
%We have used the \textbf{New York Times API} to fetch the top 10 covid news articles from the target period and display them on the panel with the period highlights. The API provides us with the flexibility to search news based on any keyword specified. We have written a Python script that sends the API the start and end dates of the user-specified target period, the search query, the number of articles to fetch, and the type of materials to view. The API returns the necessary articles based on the inputs provided. Users can scroll through the different news headlines, and by clicking on one, they can read the full article on the New York Times website.

%The entire calculation is done on the back-end using a python code.
\vspace{5pt}

\noindent \underline{\textbf{Data Cleaning}}: Raw data sets contain noise in the form of missing/incomplete values or garbage values (e.g. incomplete zip codes or state codes, ...), type or range constraint violation (e.g. string instead of integer, year range overflow, ...), attribute format issues (e.g. date and time formats not in sync for different rows) and so on. Thus, it becomes extremely important to clean the data properly in order to overcome such issues so that it does not lead to roadblocks while analyzing and avoid misleading results. Scripts are written as a part of this component to implement the different constraints for datatype, range, date-time format and so on. For CoWiz, the appropriate data sets are downloaded every 6 hours from WHO and CDC to compute the cumulative number of cases and deaths on a world/US-state basis. However, due to \textit{asynchronous updates from various agencies}, few case/death count values may not have been updated from the previous download. Thus, the data cleaning component executes a \texttt{value-constraint} check to verify whether the new count is greater than the previous count or not, and generates a \textbf{consistent cumulative case and death count file.}
    
\vspace{5pt}


\noindent \underline{\textbf{Data Modeling}}: Graphs, multilayer networks, sets, lists, files, multidimensional arrays, tensors and database relations are few of the modeling techniques that are available as a part of this component. Depending upon the objective requirements, the following data models or data structures have been utilised for CoWiz.

For \textbf{Category II objectives}, there is a need to visualize how different feature values for the US states have changed over time in the pandemic and understand the relation between them, if any. For instance, number of vaccinations vs. number of trips (\ref{C2-v2-1}, mobility in public areas vs. number of hospitalizations  (\ref{C2-v2-2}, and number of cases vs. number of tests (\ref{C2-v2-3}. For this, the \textit{clean data collected from multiple sources} (sources (\textbf{D1}) to (\textbf{D4}) listed above) is \textbf{consolidated into a single csv file} such that each row corresponds to the set of feature values (\textit{cases, deaths, vaccinations, hospitalizations, tests, population staying at home, trips more than 500 miles from home and mobility in a public areas like grocery, parks and recreational places, workplaces} and so on) for a particular state on a given date, starting from February 1, 2020.
  
  
\begin{wrapfigure}{r}{0.6\columnwidth}
\centering
%\vspace{-30pt}
\includegraphics[width=0.6\columnwidth]{figures/MLN-covid-v3}
\vspace{-20pt}
\caption{Homogeneous and Heterogeneous MLNs}
\vspace{-20pt}
\label{fig:MLN-covid}
\end{wrapfigure}
        

For \textbf{Category III and IV objectives}, the multiple relationships/interactions (similarity of cases in different periods, similarity of population density, ...) among multiple types of entities (US counties, institutions, ...) need to be analyzed. \textbf{Multilayer networks (or MLNs)} have been proposed in the literature to be an important alternative for \textit{flexible, expressive, and structure-preserving} modeling as well as efficient for analyzing complex data sets based on different combinations of features \cite{MultiLayerSurveyKivelaABGMP13,shi2017survey,ER/KomarSBC20}. MLN model is a  \textit{network of networks}. In this case, every layer represents a distinct relationship among entities with respect to a single feature. The sets of entities across layers, which may or may not be of the same type, can be related to each other as well. %Formally, a {\bf multilayer network}, $MLN (G, X)$, is defined by two sets of graphs: i) The set $G = \{G_1, G_2, \ldots, G_N\}$ contains graphs of N individual layers, where $G_i (V_i, E_i)$ is defined by a set of vertices, $V_i$ and a set of edges, $E_i$. An edge $e(v,u) \in E_i$, connects vertices $v$ and $u$, where $v,u\in V_i$ and ii) A set $X =\{X_{1,2}, X_{1,3}, \ldots, X_{N-1,N}\}$ of bipartite graphs. Each graph $X_{i,j} (V_i, V_j, L_{i,j})$ is defined by two sets of vertices $V_i$ and $V_j$, and a set of edges (also called links or inter-layer edges) $L_{i,j}$, such that for every link $l(a,b) \in L_{i,j}$,  $a\in V_i$ and $b \in V_j$, where $V_i$ ($V_j$) is the vertex set of graph $G_i$ ($G_j$.) 


Based on the type of relationships and entities, multilayer network can be of different types. The layers, nodes, intra- and inter-layer edges are decided based on the analysis requirements.

\begin{enumerate}
    \item Layers of a \textbf{homogeneous MLN (or HoMLN)} are used to model the diverse relationships that exist among the \textbf{same type of entities}. \ref{C2-1} to \ref{C4-1} need to analyze the diverse relationships that exist among the \textit{same set of US counties}. For Category III, the \textit{time periods} centered around the event of interest leads to the generation of a layer (using source (\textbf{D6}))where the nodes (US counties) are connected if there is a \textit{similar} percentage change in the number of new cases in the latest period as compared to the earlier period (Fig.\ref{fig:MLN-covid}(a).) Similarity in demographic information (from US Census data (\textbf{D7})) of counties (population, income, ...) lead to the generation of more homogeneous layers.
    %Thus, in each separate layer the US counties (nodes) are connected based on similar number of confirmed covid cases in a period, population density, traffic movement, spending categories, per-capita income and so on (Fig.\ref{fig:MLN-covid}(a)).
    \item Objectives, such as \ref{C4-3} that need to analyze the relationships among \textbf{different types of entities} like US counties (connected based on geographical proximity) and institutions like universities and MNCs (connected if have similar average number of employees (or students and staff) across branches) can be  modeled using \textbf{heterogeneous MLNs (or HeMLNs).} The inter-layer edges represent the relationship across layers (office/branch location) as shown in Fig.~\ref{fig:MLN-covid}(b). %In addition to being collaborators, researchers may be Facebook friends. Thus, to model multi-feature data that capture \textbf{multiple relationships within and across different types of entity sets}, a combination of homogeneous and heterogeneous MLNs is used, called \textbf{hybrid MLN (or HyMLN).} 

\end{enumerate}

%The choice of a data model is determined by the data set description and the analysis objectives at hand. For the Statistical Analysis and Visualization of \textit{Raw Data} (Category I), the daily data points (cases, deaths, vaccinations, ...) either need to be plotted on using line curves to understand the rise or decline (\ref{C1-1}, \ref{C1-2}) or a regression model for determine the upcoming peak (\ref{C1-3}).  Thus, for the first two categories, the data from the raw data files needs to plotted, as per the requirement and no explicit data model is required.

%\section{}


\noindent \underline{\textbf{Analysis Configuration File Generation}}: Using the user inputs as \textit{parameters} and the required data model storage paths (\textit{consistent consolidated files, set of news articles (source (\textbf{D5})) and/or MLN layers}, in case of CoWiz), a configuration file is generated and passed on to the Analysis Module, specifying the \textit{analysis expression} that need to be computed.


